Hypothesis Formalization: Empirical Findings, Software Limitations, and Design Implications

Data analysis requires translating higher level questions and hypotheses into computable statistical models. We present a mixed-methods study aimed at identifying the steps, considerations, and challenges involved in operationalizing hypotheses into statistical models, a process we refer to as hypothesis formalization. In a formative content analysis of research papers, we find that researchers highlight decomposing a hypothesis into sub-hypotheses, selecting proxy variables, and formulating statistical models based on data collection design as key steps. In a lab study, we find that analysts fixated on implementation and shaped their analysis to fit familiar approaches, even if sub-optimal. In an analysis of software tools, we find that tools provide inconsistent, low-level abstractions that may limit the statistical models analysts use to formalize hypotheses. Based on these observations, we characterize hypothesis formalization as a dual-search process balancing conceptual and statistical considerations constrained by data and computation, and discuss implications for future tools.

==> acknowledgements.tex <==
\section{Acknowledgements}

Philip Garrison and Manaswi Saha for their perspectives and feedback on our
qualitative approaches. 

==> analysis_scraps.tex <==
\begin{comment}
   TODO!! 
\textbf{API and GUI Organization.}

The breadth of linear models that the software tools support range from glmmTMB,
which was designed for count data where there are many zeros, to SPSS, which was
designed for many diverse domains and users. Thus, observations about API and
GUI organization focus on the Python libraries and interactive packages but
can also be found in the R libraries to a lesser extent. 

The software tools employed different strategies for grouping and organizing the
breadth of linear models in their APIs and GUIs. Simple linear models (e.g.,
bivariate analyses and ANOVAs) were often separated from more complex ones that
involved more specification. 

In the Python libraries and interactive packages, the more complex linear models
appeared to be grouped into subsets based on widely accepted groupings in
statistics and implementation similarity.

How many different tabs for each model -- what were they? what order? Declarative? 

Organization - Hierarchical (nested); end-user have to pick the correct linear
model (type - regression vs. Generalized Linear Model) and subtype under that;
vs. everything is flat
n
Stages of analysis - interactive packages collapse into one, eve including
visualization. JMP prides itself for the vis that it produces...


Takeaway: The packages were organized according to computational similarities more than conceptual ones? 
--> Our work does not address how to organize these things better...

Some of these organizational choices impacted the programming idioms. 
\end{comment}


\begin{comment}    
\textbf{Organization/Mixed-Effects.}
\begin{comment}
The space of linear models that are mathematically feasible and useful for
answering data analysis questions is vast. Statistical packages/libraries
provide APIs that order this vast space by utilizing specific \textit{abstractions}. In
designing an API, a library designer needs to make several design decisions
related to language abstractions: What is the appropriate \textit{level} of
abstraction? What are the \textit{primitives}? How transparent should the
underlying \textit{implementation} be?
\end{comment}

- How are the functions named differently? 
- Names and organization of APIs based on experimental design (mixedlm?)

\todo{How are models organized in interactive packages?}

There was no consistent organization of the vast space of linear models (e.g.,
regression models, generalized linear models, mixed-effects models, etc.) Tools
we analyzed consistently ordered the vast space of linear models to funnel
end-users towards a specific type and eventually instantiation of that
particular model. However, tools differed in the organizational hierarchies they
employed. 

The R libraries were more specific in scope than the Python libraries. The R
libraries were for linear mixed models (lme4) with certain kinds of data
(glmmTMB) and implementations (MCMCglmm) whereas the Python libraries included a
wider array of statistical tests, even beyond linear modeling. This difference
in scope is likely due to the fact that R is a domain-specific language for
statistical analysis with a mature ecosystem of libraries for specific aspects
of analysis whereas Python is a more general purpose language that has more
recently gained traction as a language for data analysis.

Different functions or just one where the parameters are different

Even beyond differences in scope, we identified two/three? different
organizational patterns among the software tools in our sample. Libraries either
expected end-users to know a priori the specific \textit{type} of linear model
they wanted to conduct (e.g., ) or the \textit{class} of models (e.g., linear
mixed-effects model, regression, etc.) or...

OLS vs. linear model where OLS is an option -- is this more than function naming, though?

How would even know to use the R library for instance

\ej{Is it only JMP that offers a "Fit Y By X"-like options??}

Tools required end-users to call entirely different functions for
mixed models. For example, scipy provides a mixed effects function call
\texttt{mixedlm()} that takes the dependent variable and fixed effects variables
as a formula and random effects variables as additional group parameters: \\
\texttt{mixedlm("TestScore ~ IQ", data, groups=data["Grade"])}. 

How does this organization affect/imply/hint end-users towards a mental model or
understanding of the space of linear models. What does the organization
emphasize, de-emphasize. What assumptions does the organization make or early
commitments (what happens if user doesnt search the breadth of the options
first?)

Similarly, in statsmodels,....  -- transition into catgorical variables encoding
\end{comment}


\begin{comment}
    \textbf{Organization/Mixed-Effects.}

The space of linear models that are mathematically feasible and useful for
answering data analysis questions is vast. Statistical packages/libraries
provide APIs that order this vast space by utilizing specific \textit{abstractions}. In
designing an API, a library designer needs to make several design decisions
related to language abstractions: What is the appropriate \textit{level} of
abstraction? What are the \textit{primitives}? How transparent should the
underlying \textit{implementation} be?

- How are the functions named differently? 
- Names and organization of APIs based on experimental design (mixedlm?)

\todo{How are models organized in interactive packages?}

There was no consistent organization of the vast space of linear models (e.g.,
regression models, generalized linear models, mixed-effects models, etc.) Tools
we analyzed consistently ordered the vast space of linear models to funnel
end-users towards a specific type and eventually instantiation of that
particular model. However, tools differed in the organizational hierarchies they
employed. 

The R libraries were more specific in scope than the Python libraries. The R
libraries were for linear mixed models (lme4) with certain kinds of data
(glmmTMB) and implementations (MCMCglmm) whereas the Python libraries included a
wider array of statistical tests, even beyond linear modeling. This difference
in scope is likely due to the fact that R is a domain-specific language for
statistical analysis with a mature ecosystem of libraries for specific aspects
of analysis whereas Python is a more general purpose language that has more
recently gained traction as a language for data analysis.

Different functions or just one where the parameters are different

Even beyond differences in scope, we identified two/three? different
organizational patterns among the software tools in our sample. Libraries either
expected end-users to know a priori the specific \textit{type} of linear model
they wanted to conduct (e.g., ) or the \textit{class} of models (e.g., linear
mixed-effects model, regression, etc.) or...

OLS vs. linear model where OLS is an option -- is this more than function naming, though?

How would even know to use the R library for instance

\ej{Is it only JMP that offers a "Fit Y By X"-like options??}

Tools required end-users to call entirely different functions for
mixed models. For example, scipy provides a mixed effects function call
\texttt{mixedlm()} that takes the dependent variable and fixed effects variables
as a formula and random effects variables as additional group parameters: \\
\texttt{mixedlm("TestScore ~ IQ", data, groups=data["Grade"])}. 

How does this organization affect/imply/hint end-users towards a mental model or
understanding of the space of linear models. What does the organization
emphasize, de-emphasize. What assumptions does the organization make or early
commitments (what happens if user doesnt search the breadth of the options
first?)

Similarly, in statsmodels,....  -- transition into catgorical variables encoding


==> checkpoint_06_22.tex <==
\section{Overview of project}
Overall, the project has two overarching goals: (a) to describe the hypothesis
formalization process and (b) to identify user needs and opportunities for
tools to better support hypothesis formalization. The project consists of three
investigations: a content analysis of published literature, a lab study with
data analysts, and an analysis of software tools. In line with the project's
goals, there are two main outcomes: (i) a description of the main steps involved
in hypothesis formalization and (ii) a set of design implications for
statistical software. 

\section{Content Analysis (Abbrev.)}

\subsection{Goal and Motivation}
The goal of the content analysis is to identify the stages involved in
hypothesis formalization that researchers find important to report.

\subsection{Methods (Overview)}
We randomly selected 50 publications across five different domains and conducted
a content analysis. The content we are interested in are stages involved in
hypothesis formalization (e.g., research questions, hypotheses, proxy
definition, etc.). Because the content is abstract and implicit (e.g., research
questions are sometimes implied in a discussion of related work), we conducted
multiple rounds of open coding to identify an analysis methodology and develop
an initial code book. After two rounds of revision, we finalized a code book,
which we used to code and analyze the corpus. 

More details can be found in~\autoref{sec:litSurvey}.

\subsection{Results (Briefly)}
The main outcome of the content analysis will be a discussion of the frequency
of content types (i.e., codes) and of emergent patterns in the hypothesis
formalization process (i.e., co-occurrence of codes). I am still in the process
of (re-)coding with the final code book, so I do not have any results yet, just
some preliminary observations from my previous round of coding

An observation I have made thus far is that researchers often have several
smaller hypotheses that answer a research question or an overarching hypothesis.
Hypotheses occur frequently and play different roles. For instance, researchers
may pose alternative hypotheses to check the robustness of primary findings.
Furthermore, researchers often restate the same hypothesis with greater
specificity, using proxies and statistical language (e.g., ``comparison'',
``greater effect'') the closer to the main methods or analysis section they are
stated. This funneling structure is indicative of the hypothesis formalization
process. (and the design process's fan and flare!)

Additionally, researchers do not appear to always explicitly differentiate hypotheses
from conceptual models. Conceptual models are implicit in hypotheses. However,
interestingly, conceptual models seem to appear more explicitly to contextualize
and connect statistical results, suggesting that statistical analyses reflect
and refine conceptual models. 

Overall, we find empirical evidence that broadly supports McElreath's
three-stage theoretical framework for statistical analysis that includes a
hypothesis, process (or causal) model, and statistical model. The content
analysis results also provide more granular detail than McElreath's theoretical
framework. 

An important limitation of the content analysis is that how researchers write
about their hypothesis formalization process is heavily edited to meet
scientific publication norms. The lab study helps us address and overcome this
limitation by observing analysts formalize their hypotheses in-situ. 


% The codebook is a valuable outcome of the content analysis process as it
% identifies common stages of the hypothesis formalization process.


\section{Next steps}
To finish this portion of the project, I need to (i) finish re-coding the papers
in our corpus with the finalized code book, (ii) count the occurrence of codes,
(iii) identify co-occurrences and other interesting patterns, and (iv) write
these findings up. 

\section{Lab Study (Abbrev.)}

\subsection{Goal and Motivation}
The lab study has three goals: (i) validate and build on our content analysis
findings, (ii) extend McElreath's framework to include a fourth computational
stage, and (iii) identify how software tools may affect hypothesis
formalization. Goals (i) and (ii) are in line with our larger goal of describing
hypothesis formalization (Goal a, above). Goal (iii) addresses our goal of
identifying user needs and opportunities (Goal b, above).

\subsection{Methods (Overview)}
We conducted lab studies with 24 data analysts, most of whom self-reported
substantial experience with data analysis. The lab studies included two lab
sessions and a take-home assignment. 

Given that we found empirical evidence for McElreath's general framework of
statistical analysis~\cite{mcelreath2020statistical} in the content analysis, we
structured the study tasks to mirror these phases. We added a take-home
implementation phase to help us extend the framework with the computation phase
(Goal ii). 

All lab sessions were recorded and automatically transcribed using Zoom. The
researcher also took extensive notes during lab sessions.

The researcher thematically analyzed the transcriptions and notes with the study
goals in mind. 

More details can be found in~\autoref{sec:inLabStudy}.

\subsection{Results (Briefly)}
From thematically analyzing lab session transcriptions and researcher notes, we
will uncover themes that describe (i) what data analysts do (e.g., change
hypotheses, clean data) and consider/think about (e.g., causal vs. correlation,
measurement and proxies) during hypothesis formalization; (ii) where the lab
study's structure is at odds with daily practice; and (iii) how software tools
may influence hypothesis formalization. Both (i) and (ii) findings are important for
ensuring our description of the hypothesis formalization process is external
valid.  

I am in the process of thematically analyzing transcriptions and notes from
participants who have completed both lab sessions. Thus far, I have noticed that
data analysts think about statistical implementation and mention and use
statistical software throughout the process of hypothesis formalization,
suggesting that software may influence hypothesis formalization beyond just
implementation. Additionally, it appears that analysts revise and iterate on
their conceptual hypotheses, conceptual models, and statistical models jointly,
allowing each to influence the others. Still, some data analysts are also
resistant to specifying conceptual models because they think that by explicitly
stating their assumptions and conceptual models, they will bias the statistical
analysis process.

% Surface-level categorization of problems -- could we push data scientists to engage more deeply with the domain? 
% Perhaps this is where domain expertise comes in and advantage of domain expertise to data science?

% notion of statistical information gain?

% Intermediate and analysis output could support causal model/deeper structure in
% analyses -- RQ: What is the data structure for representing these states and/or changes...?

\subsection{Next steps}
To finish this portion of the project, I need to (i) finish conducting final lab
sessions, (ii) continue to thematically analyze all transcriptions and notes,
(iii) write up results, and (iv) iterate multiple times. 

\section{Software Tools Analysis (Abbrev.)}

\subsection{Goal and Motivation}
The tools analysis aims to identify ways in which software tools implicitly
influence hypothesis formalization (Goal b, above). 

\subsection{Methods (Overview)}
We identified a set of widely used statistical libraries and GUI-based tools
following recommendations from online data science communities. After a couple
rounds of open-ended analysis, we developed a set of characteristics to pay
attention to for all tools. For each tool, we took notes as we examined articles
published about the design and implementation, API documentation and reference
manuals, and source code when available. We also took notes when completing
online tutorials and analyzing sample data with the tools. 

\subsection{Results (Briefly)}
The main finding is that current statistical software do not support or
structure the hypothesis formalization process. Tools require end-users to
specify a complete statistical model at once, even though data analysts in our
lab studies rarely did this. Furthermore, end-users must keep track of any
higher-level conceptual models or hypotheses they may have, making return visits
to analyses difficult, even though this appears to be common in practice (from
lab study interviews).

More information about the methods used in the tools analysis and its results
can be found in~\autoref{sec:toolsAnalysis}.

\subsection{Next steps}
I have not touched the tools analysis since I completed it a few months ago.
Once the results of the content analysis and the lab study are more final, I
want to revisit the tools analysis. I may want to add more tools based on the
other parts of the project and make new observations in response to the other
findings. 

\section{Discussion: Tying Three Together}
The three parts of the project complement one another in achieving our goals of (a)
characterizing the hypothesis formalization process and (b) identifying shortcomings
of existing tools and opportunities for designing new tools that support
hypothesis formalization. 

Taken together, our findings suggest a more granular and extended framework that
extends McElreath's (outcome i). The results also suggest a set of design implications (outcome ii) for
tools to support analysts in formalizing their hypotheses, or distilling
high-level hypotheses into computed statistical analyses. Furthermore, given the
differences between how researchers report their hypothesis formalization
process and how analysts go about formalization in practice, our findings suggest the
need for tools that support more complete or accurate reporting of the
hypothesis formalization process. Although not the focus of this paper, these
findings can serve as motivation for a future project (i.e., Melissa's senior
thesis). 

% design experiments with statistical analysis

\subsection{Next steps}
To develop our extension of McElreath's framework, I need to (i) finish the
other findings sections, (ii) create a diagram of how these findings fit
together, (iii) iterate on this, and (iv) draw/write it up. To develop design
implications, I need to (i) finish the other findings sections, (ii) identify
major design themes, (iii) sketch out concrete examples of tool re-designs and
new tool ideas, and (iv) write these all up. 




==> conclusion.tex <==
\section{Conclusion}

% Jeff: 
% try to define what “hypothesis formalization” is, 
% why it matters (what is at stake?), and 
% what specific challenges or pitfalls analysts face when doing it
% (whether arising from themselves, the domain, or their tools). 

Hypothesis formalization is a dual-search process of refining and translating
conceptual hypotheses into model implementations, which also involves iterative
computational refinement. Due to constraints imposed by domain expertise, data,
and tool familiarity, the same conceptual hypothesis may be formalized into
different model implementations. The same model implementation may also formalize
two possibly opposing hypotheses. Understanding hypothesis formalization enables
us to identify when and why these differences arise, which may help diagnose
reproducibility issues. While formalizing hypotheses, analysts incorporate
insights from their domain and exploratory data analysis; draw from their personal
taxonomies of statistical approaches, which may be incomplete; and rely on their tools,
which direct focus to computational details. Our findings suggest opportunities
for future tools to bridge steps involved in hypothesis formalization and guide
analysts towards reasonable model implementations. Possibilities include connecting model implementations
to their mathematical representations through meta-libraries,
providing higher-level abstractions for more directly expressing conceptual
hypotheses, and supporting automated conceptual modeling. 

==> contributions.tex <==
\figureOverivew
% \ej{Bubble up and constrain both directions? Pathways to change conceptual hypothesis because of implementation constraints and vice versa.}
\section{Contributions and Definitions}
Our work addresses two gaps in the current literature about data analysis.
First, despite the need to translate conceptual hypotheses into concrete
statistical analyses in data analysis, the process remains ambiguously defined
and \textbf{implicit} in empirical work describing data analysis.  Second,
research on statistical thinking~\cite{wild1999statisticalThinking} has shown
how statistical and domain knowledge are involved in operationalizing conceptual
hypotheses. Yet, no work engages with the role and \textbf{impact of
computation} in translating hypotheses despite the impact computational tools
have had on statistics.
%  Given the sizable impact impact
% statistical computing tools have had on data analysis, the current literature's
% oversight on the role of computation is significant~\cite{}. 

In this work, we make \textbf{explicit} the process of translating conceptual
hypotheses and define it as \textit{hypothesis formalization}. We define
hypothesis formalization as dual-search process~\cite{klahr1988dual} that
involves developing and integrating cognitive representations from two different
perspectives, that of conceptual hypotheses and of computed model
implementations. Analysts move back and forth between conceptual and
implementation spaces during formalization while navigating conceptual,
data-based, statistical or mathematical, and implementation constraints.

To ground the paper, we provide an overview and definition first. The content
analysis, lab study, and analysis of tools informed one another and our
definition of hypothesis formalization, summarized in
Figure~\ref{figure:overview}.

We characterize hypothesis formalization by contributing:
\begin{itemize}
    \item an enumeration of steps involved in hypothesis formalization (content analysis in~\autoref{sec:litSurvey}, lab study in~\autoref{sec:inLabStudy}),
    \item an identification of considerations that arise during hypothesis formalization  (content analysis in~\autoref{sec:litSurvey}, lab study in~\autoref{sec:inLabStudy}),
    \item a heuristic analysis of statistical tools and how their designs support or hinder hypothesis formalization (analysis of tools in~\autoref{sec:toolsAnalysis}), 
    \item a framework integrating the above three insights that situates hypothesis formalization in theoretical models of scientific discovery as problem solving (Figure~\ref{figure:methods}, discussion in~\autoref{sec:discussion}), and
    \item a set of implications based on the above empirical findings to inform the design of new statistical software (implications in~\autoref{sec:implications}).
\end{itemize}

By defining and characterizing hypothesis formalization, we aim to advance the
discourse around data analysis, understand how people conduct data analysis more
precisely, show opportunities for more transparent documentation towards the
reproducibility of analyses, and inform future tools that support end-users in
performing and engaging with their analysis processes.


==> discussion.tex <==
\section{General Discussion} \label{sec:discussion}
% Example Discussion: https://d1wqtxts1xzle7.cloudfront.net/45050683/The_problem_of_problem_spaces_When_and_h20160424-20767-tzaldn.pdf?1461543269=&response-content-disposition=inline%3B+filename%3DThe_problem_of_problem_spaces_When_and_h.pdf&Expires=1598892614&Signature=YztOlTxelppK7n-DtBQOc3MOUNC9Tg7ifw-h2tlTPJyDj8uskLU-FSWfiKW8EebBr7xWs~wTCmerqdDkOlwF43P3HdWxaNrVlY7-Mer84pjtEYTWUcmWbWJaZceJn-~H3DzdAkMY3HVpylAnDp07donf1dZ4Qf3uMML1C~61Bv90f9fWbKwGQBPGdIuNiY0P81wyCwhpngwADcAFX-5EGotJ1L1X-JmkuGKmrVpFDtT8CI1AVtpPYcpOxuy9Rje4MRo8Xn8ZEb-QRtlxYDXeUM29k7cG1vgYpTu9Vxuvb8Ki98aG5YMyH5l~~0gzoHDwYU76U-MFbnaFdDxKVONNaQ__&Key-Pair-Id=APKAJLOHF5GGSLRBV4ZA

% Three criteria Schunn and Khlar propose for determing spaces in problem solving:
% logical, empirical, and implementational~\cite{schunn1996and}. To justify our choice of a three space
% model, we discuss each of the spaces and the supporting evidence from the three
% investigations. 

% We situate hypothesis formalization in the larger problem solving process of
% scientific discovery~\cite{klahr1988dual,schunn1995FourSpace}. Here, we
% synthesize evidence from our literature survey, lab study, and analysis of tools
% that supports this characterization.

As a dual-search process between conceptual hypotheses and model
implementations, hypothesis formalization requires analysts to engage in problem
solving strategies characteristic of the larger scientific discovery
process~\cite{klahr1988dual,schunn1995FourSpace}. 

Hypothesis formalization involves \textit{hypothesis refinement}, which, to use
Schunn and Klahr's language~\cite{schunn1995FourSpace}, is a \textit{scoping}
process. In the content analysis, we found that researchers \textit{decomposed}
their research goals and conceptual hypotheses into specific, testable
sub-hypotheses and \textit{concretized} constructs using proxies, born of theory
or available data. Corroborating these findings, we found that analysts in the
lab study also quickly converged on the need to specify established proxies or
develop them based on the data schema presented. In hypothesis formalization,
scoping incorporates domain- and data-specific observations to qualify the
conceptual scope of researchers' hypotheses. In other words, hypothesis
refinement is an instance of \textit{means-end
analysis}~\cite{newell1972humanProblemSolving}, a problem solving strategy that
aims to recursively change the current state of a problem into sub-goals (i.e.,
increasingly specific objectives) in order to apply a technique (i.e., a
particular statistical model) to solve the problem (i.e., test a hypothesis). 

The other endpoint of hypothesis formalization, \textit{model implementation},
also involves iteration. Through our analysis of software tools, we
found that analysts must not only select tools among an array of specialized and
general choices but also navigate tool-specific taxonomies of statistical
approaches. These tool taxonomies may both differ from and inform analysts'
personal categorizations, potentially explaining why analysts in our lab study
relied on their personal taxonomies and tools. By relying on taxonomies or
familiar steps, based on previous projects or familiar tools, analysts engage in
\textit{analogical} reasoning~\cite{holland1989induction}, finding parallels between the present analysis
problem's structure and previously encountered ones or ones that fit a tool's
design most easily.

Upon selecting a statistical function, analysts may tune computational settings,
choose different statistical functions or approaches, which they may tune, and
so on. In this way, the model implementation cycle in hypothesis
formalization captures the ``debugging loops'' that analysts, such as the census
researcher in the introduction, encounter. Although the tool ecosystem as a
whole provides support for diverse model implementations, even for the same
mathematical model, the tool interfaces provide low-level abstractions, such as
interfaces using mathematical formulae, that, based on our observations in the
lab study, do not support the kind of higher-level conceptual reasoning required
of hypothesis formalization.

% How should analysts reconcile recommendations about ``conceptual simplicity''
% and best practice recommendations (e.g., Barr). Could tools help? Our model
% suggest ways for action/operationalizing these recommendations. 

% \ej{Mention visions of statistical computing futures - Breiman, Cox, Tukey?}

\begin{comment}
DISCUSSION:
- waterfall beneficial for pre-registration. However, likely that analysts
engage in iteration before pre-registering. (benefits of both approaches) 
- challenges for tools though of how to support both: tools support a workflow;
tools support portions of all workflows/overlapping pieces (which is where we
are)
\end{comment}

==> findings.tex <==

\section{Findings} \label{sec:findings}

\begin{comment}
Structure: 1. Describe High-level concept 2. Describe Axial codes 3. Explain How
do the axial codes relate to context and/or process 4. Summarize a concept --
emphasize context and process2. 
\end{comment}

\subsection{Considering a subset of all possible analyses}
We observed that end-users draw on their personal experiences and/or
observations made about smaller samples of data to develop their conceptual
hypotheses (?). In theory, a wide range of experimental design and analytical
approaches could test the conceptual hypotheses. However, end-users only
consider a small subset of all possible analyses. In this section we investigate
which analyses end-users consider and why. 

\begin{itemize}
    \item (In-lab study) TODO: Compare and contrast observations and participant
justifications between the omniscient and dataset scenarios: What analytical
decisions do participants consider when they aren't contrained by data? When
they are? 

    \item (Literature survey) Hypotheses and analyses are accretive.
Researchers often have paper-level theories they test through a series of
experiments that decompose their theories into smaller sub-hypotheses. These
sub-hypothses are often tested and modeled separately even though a larger, more
complex model could potentially provide the same information/answers.
Constraints imposed by skepticism, data availability, and experimental design
rigor seem to drive the preference for smaller sub-hypotheses. 
    
    \item (Literature survey and in-lab study) People make implicit hypotheses that
they do not necessarily treat as hypotheses. For example, researchers do not
justify why they used  linear rather than non-linear or more complex quadratic
regression models. This may be related to discipline-specific assumed,
acceptable "defaults" in a domain. 

    \item (Tools) Tools constrain the models that can
be considered by imposing model catgories that determined by implementation
details rather than end-user mental models. Programming libraries appear to
offer support for a small subset of analytical approaches, which are often
grouped together by underlying computational details. Interactive packages such
as Stata provide menus that organize models into broad categories based on data
types and gneral model structures. (This kind of reminds of the physics
education literature on how novices are fixated on surface-level similarities
between problems rather than underlying physical properties. There appears to be
a tentsion among tools for which of the two they prioritize/bubble up in their
interfaces.) 

    \item (Tools) Related to the above point, tool designers  must grapple
with reconciling model complexity with syntactical and interface simplicity,
which may be easy for expert end-users but introduces an additional barrier for
non-expert end-users.
\end{itemize}

\subsection{Encoding and trying hypotheses as mathematical models}

Trying analyses in the process of formalizing a hypothesis into a concrete
analysis is an iterative process. 

\begin{itemize}
    \item (In-lab study) TODO: Which analyses do particiapnts try and then discard or
keep? Why? What distinguishes the  iterations  for participants? (What are the
iterative patterns?)
    \item (Tools) Tools all provide support for fixed, random, and
interaction effects. However, they do not all uniformly support easy treatment
of categorical variables that might  more directly match the hypotheses
end-users have. 
    \item (Tools) Formulae is the primary vehicle through which
end-users express their hypotheses. 
    \item (Tools) There are alternatives to formulae, such as....
\end{itemize}

\subsection{Refining and choosing a concrete analysis}

\begin{itemize}
    \item (In-lab study) How do people navigate or ignore computational details? What
makes them think about them?
    \item (Tools) Tools provide support for experimenting with and customizing
    computation configurations. 
    \item (Tools) Tools provide support for debugging analyses and trying
multiple ones. (This might be too similar to the above point about
experimentation/customization.)
    \item (Literature survey) Although rsearchers reported the statistical tools
they used, they did not discuss computational configurations. As a result, if a
reader were to re-produce the analyses in another tool with different defaults,
it's not clear that the results would reproduce? (Might need to try a few. This
might be related to the above section about encoding analyses.)
\end{itemize}

==> intro_aug_03.tex <==

Data analysis is a sensemaking activity~\cite{russell1993cost}. \todo{Fill in
with examples.} In all these instances, data analysis involves continually
updating one's perspective on the motivating question and data, using statistics
as a tool in sensemaking~\cite{grolemund2014cognitive}. 

% statistics is a tool in the iterative data analysis
% process that aids one in continually updating one's perspective on the
% motivating question and problem. 
% that involves
% acquiring, manipulating, and modeling data to answer questions about the
% world~\cite{grolemund2014cognitive}.  aids in 

Along the lines of sensemaking, the American Statistics Association (ASA)
describes statistics as an ``investigative process,'' rather than the common
misconception that statistics is the rote application of mathematical procedures
to quantitative data. The ASA describes data analysis as a process that ``begins
with a question that can be translated into one or more statistical questions,''
which may be answered using visualizations, summary statistics, and inferential
statistics (see Goal 2 in ~\cite{carver2016guidelines}). Moreover, throughout
the goals the ASA outlines for rudimentary statistics education is the ability
to use statistical software to perform common tasks, such as visualization,
simulation, and...

% Separating domain-specific and
% statistical concerns is a fundamental characteristic of statistical thinking
% more generally~\cite{pfannkuch2000statistical}.
Data analysis and, statistical thinking~\cite{pfannkuch2000statistical} more
generally, involves distinguishing between \textit{domain} questions and
consideration and \textit{statistical} ones. For instance, a psychologist may
ask if women have lower annual incomes than men and then operationalize this
domain-specific question as a statistical question about the amount of variance
in differences in income between women and men gender accounts for. The
psychologist may then use a linear regression model with gender and
attractiveness as predictors~\cite{} and then interpret the results of modeling
to answer their motivating domain-specific question. 

Separating domain-specific concerns from statistical concerns and then
methodically transitioning between the two is crucial for translating
domain-specific questions into concrete statistical analyses and for
interpreting the results of statistical models to answer domain-specific
questions. We focus on the former, which we call \textit{hypothesis
formalization}. 

How do data analysts translate domain questions into statistical questions? How
do these domain and statistical questions then relate to concrete statistical
models? What is the role of statistical software in hypothesis formalization? 

% We refer to the process of distilling domain questions into concrete statistical
% models as \textit{hypothesis formalization}. 

To characterize the domain-specific, statistical, and computational
considerations involved in hypothesis formalization, this paper first develops a
framework for hypothesis formalization and then assesses the shortcomings of
current statistical tools to identify concrete ways for software could better
support hypothesis formalization. 

To understand what domain experts find important to document and communicate
about their hypothesis formalization process, we investigated a corpus of 50
research articles published in five top tier venues in domains ranging from
psychology to medicine to economics to human-computer interaction. We found that
\fillin{...}

To probe further into these considerations and patterns and identify any new
considerations or sources of information, we conducted an exploratory lab study
with 24 data analysts where we observed participants formalize hypotheses
in-situ. We found that \fillin{...}

Based on the qualitative analysis and lab study findings, we develop a
framework...

Given the importance of statistical softare in data analysis~\cite{} and that
software emerged as a theme in the formative qualitative analysis and lab study,
we analyzed 15 widely used statistical libraries and interactive packages for
how their interface and API designs may influence hypothesis formalization
(\autoref{sec:toolsAnalysis}). \fillin{Update: We found that current APIs and
GUIs require end-users to (i) have a clear statistical model they can specify
all at one time and (ii) can express their model concisely using symbolic
formulae, both of which were behaviors we did not observe in our lab study.}
Finally, given the importance of statistical softare in data analysis~\cite{}
and our observations in the lab study, we 

Taken together, the results from our content analysis, lab study, and software
tools analysis suggest three primary design implications for software tools to
better scaffold hypothesis formalization (\autoref{sec:implications}):
\fillin{list key implications.} For each design implication, we provide a
concrete example of re-designing specific aspects of existing tools or highlight
opportunities for future research and tool development. 

Overall, our characterization of the hypothesis formalization process aims to
inform data analysis practice, statistics education, and software tool
development. 



Based on these findings,....
We propose a framework that characterizes the domain-specific, statistical, and
computational considerations when data analysts formalize their hypotheses.

(ii)
operationalizing domain questions into statistical questions, (iii) constructing
statistical models to answer statistical questions, and eventually (iv)
interpreting statistical results in light of domain-specific concepts. For
instance, a sociologist may ask if women have lower annual incomes than men
(step i). They may operationalize this high-level question into a statistical
question about the amount of variance gender accounts for in models of annual
income (step ii) and then explore linear regression models that include only
gender; gender and highest education completed; or gender and
attractiveness~\cite{} as predictors (step iii). Based on the results of these
models, the sociologist may then interpret higher eta-squared values for
parameters as factors that influece income more and may be worth creating
interventions around (step iv). 


% Indeed, statistical thinking requires integrating both \textit{domain} and
% \textit{statistical} knowledge (e.g., statistical methods, modeling specifics,
% etc.)~\cite{pfannkuch2000statistical}. 



Furthermore, given the influence of software on statistics, we consider tech..

Why HCI should care. 

Although it may be tempting to attribute model exploration or choices to 
 decisions to either
statistical (e.g., avoid overfitting) computational (e.g., ensure convergence
in models) needs, 

and/or domain-specific (e.g., sociological theories,
causal models, etc. ) considerations may motivate the statistical models the
sociologist explores and the one the sociologist eventually chooses. 

Same statistical models but different interpretation based on causal models --
this is the results -> interpretation direction. We focus on the
distillation/translation of hypotheses into statistiacl models in hypothesis
formalization

For instance, consider a question....example of formalization that can lead to
different statistical models. 

Conversely, it is also possible that the same statistical model can provide
support for two different, perhaps even contradictory, hypotheses and/or causal
models. For example...

In other words, the proces of (i) distinguishing between domain questions and
statistical questions, (ii) relating them to each other, and (iii) interpreting
the results/implications of each on the other is fundamental to statistics and
data analysis. -- maybe don't mention interpretation of results, etc? We propose
the term ``hypothesis formalization'' to capture this process. 

% Despite the importance of translating domain questions and hypotheses into
% statistical questions and eventually models, 

\todo{Why should HCI researchers/CHI venue care?}

Statistics and data analysis are mediated through software tools such as...

Despite the importance of hypothesis formalization, there is little
understanding of how this process occurs. The goal of this paper is to
characterize this process by considering the cognitive, statistical, and
computational needs...\todo{Summarize methods?: by understanding hypothesis
formalization is reported in research publications, identify the constraints and
considerations involved in hypothesis formalization during data analysis, and
examine and speculate about the roles of statistical software tools in this
process.} The reason HCI reserchers should get involved is that the data
analysis process involves a mixture of cognitive and technological concerns in
addition to statistics and computation. As HCI researchers, we are uniquely
positioned to consider the cognitive, computational, and statistical demands of
data analysis, develop a multi-faceted understanding of data analysts, and
propose new interactive data analysis systems that meet this need. 

Increasingly, this statistical knowledge is also mediated by
software/statistical computing. 

To develop a broad sense of what aspects of hypothesis formalization researchers
found important to report about their process, we started with a formative
qualitative analysis involving a total of 50 research publications from
presitgious venues in five different domains. \fillin{We found that...}

To more closely observe hypothesis formalization in-situ, we designed and
conducted a lab study with 24 data analysts (\autoref{sec:inLabStudy}). \fillin{Update: Data
analysts were fixated on statistical implementation throughout, discussing
specific software and modeling techniques even while generating hypotheses
without any data, suggesting the extent to which software tools may influence
hypothesis formalization and data analysis more broadly. Analysts also relied
heavily on previous projects and sometimes struggled to reconcile the presented
scenario with past experiences or an imagined ideal data collection and analysis
scenario and tried really hard to transform the presented scenario into one that
was more familiar. We also identified a misconception that by making
hypothesized relationships about the variables in the data explicit, analysts
were biasing their analysis process. Data analysts preferred a looser connection
between their hypotheses and statistical analyses to ``let the model do the
talking,'' suggesting a tendency to conflate exploratory and confirmatory data
analysis.}

Finally, given the importance of statistical softare in data analysis~\cite{}
and our observations in the lab study, we analyzed 15 widely used statistical
libraries and interactive packages for how their interface and API designs may
influence hypothesis formalization (\autoref{sec:toolsAnalysis}).
\fillin{Update: We found that current APIs and GUIs require end-users to (i)
have a clear statistical model they can specify all at one time and (ii) can
express their model concisely using symbolic formulae, both of which were
behaviors we did not observe in our lab study.}

Taken together, the results from our content analysis, lab study, and software
tools analysis suggest three primary design implications for software tools to
better scaffold hypothesis formalization (\autoref{sec:implications}):
\fillin{list key implications.} For each design implication, we provide a
concrete example of re-designing specific aspects of existing tools or highlight
opportunities for future research and tool development. 

Overall, our characterization of the hypothesis formalization process aims to
inform data analysis practice, statistics education, and software tool
development. 

WHERE TO PUT THIS?: Data analysis requires not
only \textit{statistical} knowledge (e.g., statistical methods, modeling
specifics, etc.) but also \textit{domain} knowlege~\cite{pfannkuch2000statistical}. 


\begin{comment}
Framework? 

Move to related work?: 

Despite the importance of hypothesis formalization, little is understood about
the process. Research examining data analysts' practices have focused broadly on
data analysis tasks, overlooking hypothesis formalization entirely~\cite{}.
Existing theories of sensemaking in data analysis~\cite{} fall short of
identifying specific operations and thought patterns involved in hypothesis
formalization and do not provide implications for tools designed to more
directly support hypothesis formalization. \ej{Mention work about data analysis
troubles?} % Knowledge about hypothesis formalization is distributed/post hoc...

Use elsewhere?:
Tools do not provide support for the complex process of jointly refining
hypotheses and statistical models that we saw in the lab study. 
\end{comment}

==> limitations.tex <==
\section{Limitations}

Our investigation of hypothesis formalization focused on domain-general steps
and considerations. Domain expertise may play a significant role in how analysts
formalize hypotheses. For instance, domain experts may more quickly refine their hypotheses
and spend less time iterating on their model implementations because they are
familiar with computational settings and their conceptual and statistical
ramifications. Future work observing domain experts perform hypothesis
formalization would enrich our domain-general view. Additionally, in domains
where pre-registration has become more mainstream, such as in psychology,
future research could also examine how researchers arrive at the studies they
pre-register. Given the level of detail in some pre-registered studies,
researchers likely engage in a version of the hypothesis
formalization process we have identified here prior to registration. 

Similar to how heuristic evaluations identify usability challenges, our
heuristic analysis of software tools revealed misalignments between tool design
and the hypothesis formalization process. Follow-up user studies are necessary
to draw stronger conclusions about how the menu structures of GUIs and the
inconsistencies across APIs affect statistical understanding, for example.
Studying users in a lab or observational setting, especially over time, would
likely reveal additional implications for improving existing tools and
developing new ones. 

Although seeking additional, outside information during hypothesis formalization
was common in the lab study, information sources and collaboration are
dimensions of hypothesis formalization that we did not investigate deeply.
Based on our findings, we expect that (i) domain and data information is helpful for
refining hypotheses, (ii) tool documentation is helpful during model implementation, and (iii)
statistical information is helpful all throughout. Future work should investigate precisely
how and when different kinds of information and collaborations serve hypothesis
formalization goals.  


\begin{comment}
TO CONSIDER FOR DISCUSSION, NOT IMPLICATIONS: 
a) American Stats Association: In other words, hypothesis
formalization is considered a core competency in statistics. Therefore,
understanding and reifying how practitioners formalize hypotheses could benefit
statistics education and ultimately increase statistical literacy and thinking. 

b) Proposing a theory of data analysis is important for the continual maturation
of data analysis (similar to Gorlemund and Wickham paper). -- benefits of better
understanding hypothesis formalization

c) Wilkinson and Tukey predictions... 


Implications demonstrates utility of our model

FUTURE WORK?
1. Taxonomy as an abstraction/entry point into mathematical/statistical representation space of models. 
2. Domain knowledge, personal experimence, and data properties constitute/constrain decision making in taxonomy.
3. How the taxonomies develop is unclear, but apepars to be based on prior experiences and possibly how learned stats, including the tools used to teach stats.

\end{comment}

==> methods.tex <==
% \figureOverivew

\section{Methods}~\label{sec:methods}

% \subsection{A Note on Methods, Findings, and Organization}
We used the Grounded Theory Method (GTM) to develop our
theory~\cite{glaser1967discovery}. Since its inception, GTM has developed
different methodological and philosophical branches~\cite{muller2014GTM}. We most
closely follow the method as Corbin and Strauss
describe~\cite{corbin2008strategies}. 

We analyzed (i) statistical analysis software tools, (ii) published empirical
research articles, and (iii) the artifacts participants created during a natural
programming in-lab study. Our emergent understanding of the data guided our
sampling, which was iterative and open-ended. Coding one source of data informed
additional sampling of other sources of data (theoretical sampling).

In the end, we identified \ej{N} axial codes that comprise {3?} key concepts.
Our hypothesis formalization theory then arose out of these concepts. 

We next describe our sampling and analytical methods for each source of data.
The following section (\autoref{}) discusses the findings, organized by concept
and axial code. Because all three sources of data informed the concepts and
axial codes, we discuss the results from the three different data sources
together. 


\subsection{Software Tools Analysis}
Our primary motivation for examining the tools was to understand how tools could
implicitly impact and constrain the hypothesis formalization process through
their interfaces and implementation, such as by requiring specific ways of
expressing hypotheses or making certain kinds of hypotheses easier to express
than others. 

\textit{Sample.} 
We analyzed a total of XX tools. We analyzed both software libraries and more
interactive packages with graphical user interfaces. Table X gives an overview
of the tools. 

We started by analyzing widely adopted software tools. We identified these
through online community recommendations~\cite{grolemund2019:recommendedR,
bobriakov2017:top15Python, bobriakov2018:top20Python, prabhu2019:topPython,
rStudioTwitter, rStudioCommunity} and our experiences teaching and conducting
data analysis. While we analyzed published research articles (as described
below), we added any relevant tools mentioned in the papers to our sample.
% if they were sufficiently different from our existing sample. 

\textit{Analytical material and focus.}
To analyze the software tools, we read articles published about the libraries'
designs and implementations, read API documentation and reference manuals,
followed online tutorials to learn the tools, analyzed our own dataset with the
tools, and examined source code when available. 

On the avialable materials, the first author completed a round of open coding
and note-taking on most of the data and then followed-up with multiple rounds of
code definition and revision based on feedback from the other authors. 

Because our focus was to notice where software tools might constrain how
end-users express hypotheses, we paid attention to the following characteristics
of software tools:
\begin{itemize}
    \item the functions (and parameters) an end-user must invoke, 
    \item any programming idioms (e.g., sequence of functions) made easier with a tool, 
    \item default settings and properties of analyses, 
    \item the ease with which to change those defaults, and 
    \item statistical metrics and output that might help with hypothesis testing. 
\end{itemize}


\subsection{Published Literature Survey}
To develop an understanding of how people formalize their hypotheses and discuss
their formalization processes, we analyzed published empirical research
articles. 

\textit{Sample.}
We analyzed a total of XX published articles from diverse disciplines, including
psychology, biology, and \ej{computer science?}. Our emergent questions and
understanding guided our sampling of papers. Table XX gives an overview of the
papers and journals we analyzed. 

We identified high-impact journals in these areas using Google Scholar's
rankings which are based on h-indices for each publication venue in 2014-2018
(latest available data at the time of
writing)~\footnote{\hyperlink{https://scholar.google.com/citations?view_op=top_venues&hl=en}}.

We started open coding with a sample of six papers published in the January 2019
edition of Psychological Science. Although we did not expect any bias of
publication edition given the varying lengths of revision cycles, we aimed to
minimize any possible biases from publication edition or venue for future
samples. In case reporting procedures have changed over time, we restricted our
samples to papers published in 2015 or later.

To obtain random samples of publications, we wrote scripts to randomly sample
papers from each venue. The appendix~\autoref{sec:Appendix} includes more
information about our sampling procedure and contains links to our scripts.

\textit{Analytical material and focus.}
We analyzed the manuscripts of publised articles and, when available,
supplemental materials, including datasets and analysis scripts. 

We were particularly interested in identifying authors' conceptual hypotheses
and how they formalized them into concrete statistical analyses. Specifically,
we focused on authors' \textit{rationale} for picking the analytical strategies
they did. We were especially attuned to any \textit{implicit prioritizations}
and \textit{justifications} authors made about their analytical decisions. For
each paper, we asked the following guiding questions: 

\begin{itemize}
    \item What analytical choices are treated as important to discuss? less important? unimportant and therefore omitted?
    \item What is taken for granted? In other words, if we were to re-do the analysis as described in the paper, what is missing? 
    \item How do the analytical choices relate back to the hypotheses authors are trying to test?
\end{itemize}


\subsection{In-lab study}
Why: Limitation of the survey 

\textit{Sample.}


\textit{Method.}



\begin{comment}
A curiosity about how end-users go from high-level conceptual hypotheses to
specific statistical tests prompted our work. Through the GTM process, our
questions and insights became more multi-dimensional, and the emergent focus
throughout our sampling procedure was to understand how hypothesis formation is
structured, performed, and otherwise influenced by software tools, end-user
knowledge, data, and community expectations.

We employed theoretical sampling. Questions that emerged from our data analyses
informed our subsequent data collection processes and vice versa. Theoretical
sampling led us to integrate prior work with our own observations and analyses
from (i) the implementation and documentation of popular software tools for
statistical analysis, (ii) published research papers that conduct statistical
analyses, and (iii) in-lab studies with participants. From these sources, the
theory of hypothesis formalization emerged. 

Figure~\ref{figure:overview} gives an overview of the analysis and collection process. Although
the addition of each new source influenced theory development, significant
shifts in data collection are included in the overview. 

For the sake of readability and comprehension, we first present the theory
in~\autoref{sec:theory}. Then, we present the findings derived from the three
broad sources of data separately (i.e., tools~\autoref{sec:toolsAnalysis},
literature~\autoref{sec:litSurvey}, and in-lab
studies~\autoref{sec:inLabStudy}).~\autoref{sec:discussion} then brings the
findings from each source together for a richer discussion about the emergent
theory. Nevertheless, it is important to emphasize that juxtaposing and
intermingling the analysis and collection of these heterogeneous data sources
was crucial to developing the theory of hypothesis formalization.
\end{comment}
% GTM is characterized by two key attributes: a) data are
% analyzed as they are collected and b) the result of grounded theory analysis is
% a theory. In accordance with GTM, we analyzed data as we collected them, and our
% analyses informed our sampling methods, as discussed in greater detail in the
% sections to follow. 

    
    \begin{comment}
    GORC info is outdated now...
    What would go in the appendix: The GORC dataset is distributed in 10K batches.
    Each batch has several thousand papers. Any given paper in the dataset is
    uniformly randomly assigned to a batch. As such, we take a random sample of
    papers from a particular venue by looking through one batch at a time. We stop
    the sampling process once the desired number of papers (sample size) is reached.
    The script is available online at~\redacted. 
    \end{comment}



Preliminary, exploratory analysis to identify motivating research questions and feasibility of using published literature: 
- 6 Psych Science, 2 Nature papers
OPEN CODING: 
Psychological Science: 
- Working Memory Has Better Fidelity Than Long-Term Memory: The Fidelity Constraint Is Not a General Property of Memory After All
- Separate Contribution of Striatum Volume and Pitch Discrimination to Individual Differences in Music Reward
PNAS:
- GUN1 interacts with MORF2 to regulate plastid RNA editing during retrograde signaling
- Brain-wide genetic mapping identifies the indusium griseum as a prenatal target of pharmacologically unrelated psychostimulants
Nature: 
- Cortical pattern generation during dexterous movement is input-driven
- "A new species of Homo from the Late Pleistocene of the Philippines" Analogue quantum chemistry simulation
- "H+ transport is an integral function of the mitochondrial ADP/ATP carrier"
CHI: 
- paper148
- paper482
- paper488
- paper705
JFE: 
- The relevance of broker networks for information diffusion in the stock market
- Do firms hedge with foreign currency derivatives for employees?
- The liquidity cost of private equity investments: Evidence from secondary market transactions

==> older_files/analysis.tex <==
\section{Study 1: Analysis of existing libraries}

The space of linear models that are mathematically feasible and useful for
answering data analysis questions is vast. Statistical packages and libraries
aim to structure this vast space by creating abstractions and designing APIs for
end-users to build linear models that test their hypotheses and answer their
research questions. In designing an API, a library designer needs to make
several design decisions related to language abstractions: What is the
appropriate level of abstraction? What are the primitives? How transparent
should the underlying implementation be?

\subsection{Aim}
In this work, we aim to map the space of abstractions and design patterns linear
modeling libraries employ. 

\subsection{Approach}
We analyzed a total of XX programming libraries used for building linear and
nonlinear models for data analysis (XX in R and YY in Python).

\textbf{Identifying R packages to analyze: }As of the end of 2019, 15,365
packages were registered with the Comprehensive R Archive Network (CRAN), the
entity that manages and distributes R packages. Of the 15K packages, we scraped
279 that had both the words ``linear'' and ``model'' as substrings in the
package titles~\footnote{Scraping script included as an appendix.}. Of the 279
packages, manual inspection of the titles revealed that 270 were for building
linear models and relevant to our analysis. (Six packages were supplementary
materials for textbooks and three packages were primarily for visualization.) 

We leveraged snowball and random sampling techniques to
identify which of the 270 R packages to analyze. Based on our experiences
teaching and doing data analysis, recommendations from R
Studio~\cite{grolemund2019:recommendedR}, and sugggestions R users made in
response to posts the first author made on the R Studio Community forum and R
Statistics Twitter page asking about popular libraries for linear modeling, we
began our analysis with three libraries (i.e., lme4, brms, and glm). We
additionally analyzed three other libraries our initial set of three libraries
referenced in their manuals/documentation and published papers. \ej{I haven't
done this part yet. Not sure if it's worth doing: For increased coverage, we
then randomly sampled and analyzed an additional 21 libraries (10\% of the R
libraries available at the end of 2019 that explicilty supported linear
modeling).}

\textbf{Identifying Python packages to analyze: }Using Helena~\cite{} to scrape
the Python Package Index (PyPI) for all registered packages under the
``Scientific/Engineering' topic, we identified XX number of packages that had
``linear'' and ``model'' substrings in their package titles or project
descriptions. Taking into consideration that Python is a more general purpose
programming language than R, which therefore could encourage package authors to
summarize their packages at a higher-level (e.g. ``data analysis'' rather than
``linear modeling'), we expanded our search for relevant Python packages. We
identified an additional XX packages that used ``'' in their titles. 

Further filtering....


We took an approach similar to our approach for identifying R packages to
analyze. Based on our expereinces teaching and conducting data analysis and
recommendations from the Python data science
community~\cite{bobriakov2017:top15Python,bobriakov2018:top20Python,prabhu2019:topPython},
we started our analysis with four libraries (i.e., Statsmodels, Numpy, Scipy,
and Pandas). To increase reprsentativeness, we also randomly sampled and
analyzed an additional XX libraries found on PyPI (total of 10\% coverage of
Python libraries).

\textbf{Analysis procedure: }We inductively analyzed the R and Python libraries by reading published research
papers and online documentation about the libraries. We primarily focused on the
APIs and key design decisions, devling into library implementations when
necessary. For our analysis, we started with the following guiding questions: 
\begin{itemize}
    \item What are the abstractions the library uses? (e.g., What does the
    end-user write? What are the functions the end-user invokes?s)
    \item What are the defaults and customizations available for the following
    comprehensive, albeit not exhaustive, characteristics of linear models?: covariates, categorical variable
    encoding schemes, random effects, random effects, interaction effects, mixed
    effects, contrasts, and hyperparameters.
    \item What is the output provided back to the end-user?
    \item How does the library support non-linear models, if at all?
\end{itemize}


\section{Results}
-programming model
-primacy of formula

==> older_files/tools_analysis_old.tex <==
\section{Study 1: Analysis of existing libraries}

The space of linear models that are mathematically feasible and useful for
answering data analysis questions is vast. Statistical packages/libraries
provide APIs that order this vast space by utilizing specific abstractions. In
designing an API, a library designer needs to make several design decisions
related to language abstractions: What is the appropriate \textit{level} of
abstraction? What are the \textit{primitives}? How transparent should the
underlying \textit{implementation} be?

% End-users use these APIs and rely on
% the underlying abstractions to build linear models that test their hypotheses
% and answer their research questions. 

\subsection{Aim}
In this work, we aim to map the space of abstractions and resulting programming
models that current linear modeling libraries offer. 

\subsection{Approach}
We analyzed a total of XX programming libraries used for building linear and
nonlinear models for data analysis (XX in R and YY in Python).

\textbf{Identifying R packages to analyze: }As of the end of 2019, 15,365
packages were registered with the Comprehensive R Archive Network (CRAN), the
entity that manages and distributes R packages. Of the 15K packages, we scraped
279 that had both the words ``linear'' and ``model'' as substrings in the
package titles~\footnote{Scraping script included as an appendix.}. Of the 279
packages, manual inspection of the titles revealed that 270 were for building
linear models and relevant to our analysis. (Six packages were supplementary
materials for textbooks and three packages were primarily for visualization.) 

We leveraged snowball and random sampling techniques to
identify which of the 270 R packages to analyze. Based on our experiences
teaching and doing data analysis, recommendations from R
Studio~\cite{grolemund2019:recommendedR}, and sugggestions R users made in
response to posts the first author made on the R Studio Community forum and R
Statistics Twitter page asking about popular libraries for linear modeling, we
began our analysis with three libraries (i.e., lme4, brms, and glm). We
additionally analyzed three other libraries our initial set of three libraries
referenced in their manuals/documentation and published papers. \ej{I haven't
done this part yet. Not sure if it's worth doing: For increased coverage, we
then randomly sampled and analyzed an additional 21 libraries (10\% of the R
libraries available at the end of 2019 that explicilty supported linear
modeling).}

\textbf{Identifying Python packages to analyze: }Using Helena~\cite{} to scrape
the Python Package Index (PyPI) for all registered packages under the
``Scientific/Engineering' topic, we identified XX number of packages that had
``linear'' and ``model'' substrings in their package titles or project
descriptions. Taking into consideration that Python is a more general purpose
programming language than R, which therefore could encourage package authors to
summarize their packages at a higher-level (e.g. ``data analysis'' rather than
``linear modeling'), we expanded our search for relevant Python packages. We
identified an additional XX packages that used ``'' in their titles. 

Further filtering....


We took an approach similar to our approach for identifying R packages to
analyze. Based on our expereinces teaching and conducting data analysis and
recommendations from the Python data science
community~\cite{bobriakov2017:top15Python,bobriakov2018:top20Python,prabhu2019:topPython},
we started our analysis with four libraries (i.e., Statsmodels, Numpy, Scipy,
and Pandas). To increase reprsentativeness, we also randomly sampled and
analyzed an additional XX libraries found on PyPI (total of 10\% coverage of
Python libraries).

\textbf{Analysis procedure: }We inductively analyzed the R and Python libraries by reading published research
papers and online documentation about the libraries. We primarily focused on the
APIs and key design decisions, devling into library implementations when
necessary. For our analysis, we started with the following guiding questions: 
\begin{itemize}
    \item What are the abstractions the library uses? (e.g., What does the
    end-user write? What are the functions the end-user invokes?s)
    \item What are the defaults and customizations available for the following
    comprehensive, albeit not exhaustive, characteristics of linear models?: covariates, categorical variable
    encoding schemes, random effects, random effects, interaction effects, mixed
    effects, contrasts, and hyperparameters.
    \item What is the output provided back to the end-user?
    \item How does the library support non-linear models, if at all?
\end{itemize}


\section{Results}
-programming model
-primacy of formula 

Our approach to analysis was to focus on the most widely used packages in R and
Python. To identify such packages, we relied on online community recommendations
and our experiences teaching and conducting data analysis in both languages. 

==> proposed_lit_survey.tex <==
\section{[IN PROGRESS] Formative Study: Literature Survey} \label{sec:litSurvey}

Our objective is to understand how researchers report on the hypothesis
formalization process with an eye towards identifying the steps and decisions
that researchers explicitly discuss, implicitly mention, or omit entirely.
Towards this aim, we qualitatively analyzed \fillin{80} research publications and their
supplemental materials from \fillin{five} different domains.

\subsection{Method}

\subsubsection{Goal.}
My overall goal is to get a broad sampling of papers. I don't want to
necessarily generalize my observations to a specific venue but rather be
sensitive to common patterns across domains, noting any domain idiosyncrasies
where appropriate. 


\subsubsection{Sample.} 
My previous strategy was to sample papers from Psychological Science, Nature, and CHI
(diversity of disciplines). 

\textbf{Sampling strategy 1: }To get my feet wet and start developing a coding
strategy, I read and analyzed papers published in January 2019 in Psychological
Science. I recognized that my sample was biased (papers published in a single
year and month), I thought it might be okay since I didn't have any evidence yet
that publication date had any effect on hypothesis formalization.

\textbf{Sampling strategy 2: } When I was more focused on grounded theory, I was
trying to rely more on notions of "theoretical sampling" that prioritize testing
emergent understanding incrementally rather than getting a representative
sample, so I continued to look at papers in 2019 but began to look for papers
published in Nature. (My understanding of theoretical sampling and grounded
theory comes from Corbin and Strauss~\cite{corbin2008strategies}, one of the
many different views on grounded theory.) 

\textbf{Sampling strategy 3: }Moving away from grounded theory, I had been
``landscape sampling,'' a purposive sampling method called ``landscape
sampling,'' following the procedure described in ~\cite{Bos2007:Collaboratories}
of research papers in psychology, the life sciences, and computer sciences.
Although landscape sampling does not enable us to make conclusions about the
frequency of particular kinds of conceptual hypotheses, concrete analyses, or
justifications, the method suited our goal of widely exploring the breadth of
hypotheses and analyses researchers employ and their reasons for their choices. 

\textbf{Sampling strategy 3, adapted: }I had started sampling papers published
in 2019 only, but then I thought our findings might be more generalizable if we
analyzed papers in other years, so I have been pseudo-randomly sampling papers
from 2015 onward. 

My inclusion criteria were to include  papers that have used different
conceptual hypotheses, analyses, or justifications of analysis decisions than
others in my sample. However, I haven't found a fair proxy/definition of what a
``similar'' conceptual hypothesis, analysis, and/or justification would be to
warrant saturation/cease sampling.

To identify candidate papers to include in my landscape sample, I used a pseudo-random strategy outlined in~\autoref{sec:Appendix}.

\textcolor{red}{\textit{Pivot sampling strategy.} My observation from reading and analyzing
papers from the last five years has been that there are different reporting
trends/checklists that have been introduced, adopted, and changed publication
communities and practices, especially with respect to the reporting of findings,
statistics, and, consequently, hypothesis
formalization.~\footnote{https://www.nature.com/nature-research/editorial-policies/reporting-standards}
Thus, I think my data would be more uniform and and my analyses better suited by
a focus on 2019 papers, presumably when venues have the latest (or close to latest)
procedures/checklists in place.}

\textcolor{red}{I propose to (1) expand the set of venues I consider and (2) take a random
sample of papers from each venue. }

\textcolor{red}{\textit{Expand venues.}
Below are the venues I'm thinking of including. They are highly ranked in Google
Scholar overall and/or in their respective fields and (2) I have access to them
(open access or through UW). Other highly ranked venues are closed access, and
UW's license only gets me partial access.
\begin{itemize}
    \item Nature journal (898 research articles published in 2019)
    \item Psychological Science (139)
    \item PNAS (4028)
    \item Journal of Financial Economics (134)
    \item CHI (705, though not all are empirical/use stats!)
\end{itemize}}

\textcolor{red}{\textit{Random sampling.}
I propose to pivot from a landscape sample to a random sample of K\% (1 - 5\%?)
or N (20-40?) papers from each venue. The benefit of a percentage-based sample
is that we can get approximately the same coverage for each venue, which would
be advantageous if we think that venues with more research publications have a
greater diversity of hypotheses, analyses, and justifications. On the other
hand, our sample would be skewed towards high-throughput venues, which in this
case might be fine since those would be Nature and PNAS, venues which publish
research on diverse topics. The benefit of a count-based sample is that would
have a balanced sample and our observations are less likely to be skewed towards
certain venues. The main drawback would be that our sample would be even less
representative of more heterogeneous and less coverage of high-throughput
venues. Neither strategy is obviously advantageous. I think starting with a 1\%
random sample (or 10 papers if 1\% is less than 10) is a reasonable middle ground.}

\subsubsection{Coding.}
I have tried a few different analysis approaches and passes. They can roughly be
defined as such:
\begin{itemize}
    \item \textbf{First pass:} Read through, get a sense of what information I
could glean and where. \textit{Biggest insight:} 1) Information is distributed.
Aka. look at supplemental material. 2) Publication venues have different
reporting biases.
    \item \textbf{Second pass:} Open coding, just based on what I found in the
data. \textit{Biggest insight:} I need to incorporate codes from outside, too.
(Emic and etic coding)
    \item \textbf{Third pass:} Open coding (continued) with some
insight/guidance/codes from tools analysis. Integrating the two sources was a
particular focus and interest when I was taking a more grounded theory approach.
I was trying to figure out how to integrate the tools analysis and the
literature survey together. \textit{Biggest insight:} From the second and third
passes and another partial pass: (i) initial documentation of codes and (ii) how
to break them apart/connect with tools analysis.~\footnote{https://docs.google.com/document/d/1aq0IiA24SUNsqNqhJfQSzrWMIV3tGGhoVPGbasrrJnM/edit}
    \item \textbf{Fourth pass:} Move away from grounded theory. Focus on the
    concrete questions we want answered from the literature survey independent
    of the other data sources. \textit{Biggest insight:} Update three guiding questions, below. 
\end{itemize}

Guiding questions: 
\begin{enumerate}
    \item What are the conceptual hypotheses researchers have?
    \item What are the concrete analyses researchers use to test their conceptual hypotheses?
    \item How do researchers justify their formalization choices? Specifically, what analytical choices are treated as important to discuss? less important? unimportant and therefore omitted?
\end{enumerate}

% \tableLitSurvey 

\textcolor{red}{I think it will be methodologically cleaner and more reliable if
I start over. Given that I had so many pivots and analysis passes that I didn't
document as well as I could have, I think starting with a new sample and coding
strategy would be more sound.}

\textcolor{red}{Specifically, I'm thinking about (1) randomly sampling 1\% of papers (as
outlined above), (2) generating new open codes,  (3) creating a code book, and
then (4) going back through the data with the code book (probably will take a
few different passes).} 

\textcolor{red}{I don't think it makes sense to use open codes I have so far (from another
sample) on this new sample. I think there will be significant overlap, but I
still think it is  to start over.}

\textcolor{red}{For a more detailed explanation of my proposed steps, please see~autoref{sec:RevisedAppendix}.}




% \textit{Analytical material and focus.}
% We analyzed the manuscripts of published articles and, when available,
% supplemental materials, which included datasets and analysis scripts. We restricted
% our sample to papers published during 2015 or later to control for any temporal
% effects.

% \textit{Coding procedure.} 
% Our coding procedure was iterative. The first author started by open coding a
% sample of six papers published in the January 2019 edition of Psychological
% Science. As the sample grew, they created and used additional codes as needed.
% Throughout this process, the authors met, discussed, and revised codes
% regularly.

\subsection{Preliminary Findings}

\subsubsection{Evidence of hypothesis formalization?: Nested hypotheses}
often many more in the supplemental materials, for defining and concretizing
the hypothesis, testing confounders, etc.

Does hypothesis formalization apply to each sub-hypothesis only or to the entire
process, including the breaking down of the paper-level hypothesis into
sub-hypotheses?

\subsubsection{Absence of Mathematical Notation or Precision?}
- use of visualizations
- use of tables with parameter estimates? 

\subsection{What was consistently included} 

\subsubsection{What was consistently excluded}
- 

\subsubsection{Reasons for selecting analyses}
Consistent with prior interview studies on the motivations and rationale people
have for making some analysis decisions, prior work. 

When omitted, likely unspoken domain-specific expectations or standards.


\subsection{Limitations}
-Reported statistics may be a result of exploration dressed up as confirmation -- how do we account for this?
-Polished form of research publication is unlikely to contain all the details
that honestly depict the hypothesis formation process
-Social pressures to include statistics as rhetoric accepted in the community

What is reported in  and included in the supplemental material for a published
research article is the final, polished artifact, with histories and thorny
decisions omitted~\cite{liu2019paths}. Motivate next study: To get a more
realistic understanding in-situ, we conducted an in-lab user study. 

Implication - data provenance tracking tools? (What might those limitations be
also? )


==> supp_material.tex <==
\section{Working list of supplemental material to submit with paper}
\subsection{Literature Survey}
\begin{enumerate}
    \item Table of papers, summary, contribution types
    \item Reorderable matrices for all
\end{enumerate}

\subsection{Lab Study}
\begin{enumerate}
    \item Pre-study survey
    \item Instructions for all tasks
    \item Post-study survey
\end{enumerate}

\subsection{Tools Analysis}
\begin{enumerate}
    \item Table identifying/aggregating info about the tools
\end{enumerate}

==> tea_lm.tex <==
\section{Study 3: User Evaluation}

\subsection{Aim/Problem}

(Based on our analysis and literature survey,) We hypothesize that higher-level
linear modeling APIs that focus on eliciting end-users' hypotheses will be more
usable, faster, and more direct to answering high-level research questions and
hypotheses. 

% We aim to develop a library for linear modeling that better supports
% end-users to select linear models that more closely test their hypothses and
% research questions. 

\subsection{Implementation}

In order to test our hypothesis, we implemented an extension to Tea~\cite{jun2019tea}, a
high-level Python package for automatically selecting statistical tests.

\section{Study}

We conducted a two-hour in-lab study with 20 participants. Dataset for analysis
was between-subjects whereas tool varied within-subjects. 

Participants analyzed one of two datasets: \dots The datasets are equivalent
because \dots For each dataset (synthetic?), a researcher presented participants with two sets
of five questions (?) research questions and hypotheses to answer with each the
dataset. Participants also were encouraged to identify and answer any additional
research questions and hypotheses they wanted to ask. Participants either
completed the task with Tea or with any library of their choice. The tool order
question order was randomized across subjects to mitigate learning effects. 

We measured the accuracy of participants' conclusions and the time taken to
complete a statistical analysis and interpret the results. We also collected
survey responses about the experience using the tool. 
% What did participants find hard to use or do with the tool?

\begin{comment}
\section{User Study 2: Maybe? Depending on outcome of first two studies?}
Improving the feedback from our first user study, we conducted a second lab
study where we compared how effectively non-statistical experts could conduct
linear models using R/Python and Tea. 
\end{comment}

==> tech_requirements.tex <==

Language and interface design:
what if we could imagine an
even higher level of abstraction that (1) is at the same level as the hypotheses
and research questions that drive the analysis in the first place and (2) are
more accessible to people who may not come from statistical or mathematical
backgrounds. (Is there a reason 3??)

==> theory.tex <==
\section{Theory of Hypothesis Formalization} \label{sec:theory}

\subsection{Definitions}
\begin{itemize}
    \item conceptual Hypothesis
    \item concrete statistical analysis
\end{itemize}

It might also be helpful to provide a visual that describes our theory....
